CoreNEURON : An Optimized Compute Engine for the NEURON Simulator

The NEURON simulator has been developed over the past three decades and is widely used by neuroscientists to model the electrical activity of neuronal networks. Large network simulation projects using NEURON have supercomputer allocations that individually measure in the millions of core hours. Supercomputer centers are transitioning to next generation architectures and the work accomplished per core hour for these simulations could be improved by an order of magnitude if NEURON was able to better utilize those new hardware capabilities. In order to adapt NEURON to evolving computer architectures, the compute engine of the NEURON simulator has been extracted and has been optimized as a library called CoreNEURON. This paper presents the design, implementation and optimizations of CoreNEURON. We describe how CoreNEURON can be used as a library with NEURON and then compare performance of different network models on multiple architectures including IBM BlueGene/Q, Intel Skylake, Intel MIC and NVIDIA GPU. We show how CoreNEURON can simulate existing NEURON network models with 4-7x less memory usage and 2-7x less execution time while maintaining binary result compatibility with NEURON.

==> tex/modeling.tex <==
%Describe use cases and workflows (Francesco to provide)
%What is it we want to simulate ?  
In this study focus is given on \emph{hybrid clock-event driven simulations of compartmental models of spiking neural networks}, using the NEURON software as a representative implementation. \par


Compartmental models of neurons take into account not only the connectivity between neurons but also the individual morphologies and inhomogeneities of each neuron. As such, they model each neuron as a set of lines, called \emph{sections}, connected at their ends through branching points. Each section can have its own set of biophysical parameters, independently from other sections, and is discretized as a set of adjacent segments of equal length, called \emph{compartments} (see e.g.~\cite{hines1993neuron}). \par

The electrical activity of neurons is modeled using the cable equation (see e.g.~\cite{tuckwell2005introduction}) applied to each section, where the quantity representing the state of a neuron at a given point in space and instant in time is the \emph{membrane potential}. The membrane potential can be affected by three phenomena:
\begin{enumerate}
\item A passive reaction-diffusion component arising from the cable approximation
\item An active reaction component arising from the presence of particular proteins on the membrane, \emph{ion channels} also referred as mechanisms, who typically have complex nonlinear interactions with the membrane potential
\item An event driven component arising from the presence of synaptic events, a feature that allows neural neurons to communicate by releasing chemical species in the extracellular space neighbouring synapses (also referred as mechanisms) of other neurons
\end{enumerate}
\par
Hybrid clock-event driven simulations are implemented in the following way: the first two elements of the previous list are resolved via standard ODE approximation techniques, such as finite differences (see e.g.~\cite{mascagni1989numerical}); whereas the last one is implemented via a queue of events (ordered by delivery time) that will prompt the execution of a callback function (see~\cite{brette2007simulation} for a complete review).

The general form of the cable equation for a section, in the case of constant parameters and conductance based synapse modeling, is given by:
\begin{equation}\label{eq:cable}
\frac{d}{2L^2R_a }\frac{\partial^2 v}{\partial x^2} = c_m\frac{\partial v}{\partial t} + I_{pas} + I_{ion} + I_{syn}
\end{equation}
where
\begin{itemize}
\item $\displaystyle d \left[\mu m\right] , R_a \left[\Omega cm\right], c_m \left[\frac{\mu F}{cm^2}\right], I_{pas}=g_{pas}(v - e_{pas}) \left[\frac{nA}{cm^2}\right]$ are biophysical parameters contributing to the passive component of the cable equation;
\item $\displaystyle I_{ion} = \sum\limits_{i=0}^{N_{ion}} g_i(v - e_i)~\left[\frac{nA}{cm^2}\right]$ is the active contribution arising from ion channels along the section, whose conductances $g_i$ and resting potentials $e_i$ might depend in a nonlinear fashion upon a set of state variables representing those channels;
\item $\displaystyle I_{syn} = \sum\limits_{j=0}^{N_{syn}}g_j(v - e_j)\delta(x - x_j)~\left[\frac{nA}{cm^2}\right]$ is the contribution from the synapses placed at positions $x_j$, whose conductances $g_j$ and resting potentials $e_j$ might depend in a nonlinear fashion upon a set of state variables and which take effect in a strongly localised manner as a consequence of the presence of the Dirac delta function $\delta(x - x_j)$;
\end{itemize}
As stated before, one needs to couple~\eqref{eq:cable} to a set of additional differential equations that describe the evolution of the states of ion channels and synapses, thus giving rise to a system of PDEs/ODEs as the final problem.\par
A widely used method of discretizing~\eqref{eq:cable} and solving the corresponding linear system is known as the Hines algorithm, and has been introduced in~\cite{hines1984efficient}. The high order of accuracy and stability of this method make it the de facto standard in the neuroscientific community. \par 
The general structure of a hybrid clock-event driven algorithm making use of the Hines algorithm can then be divided in six phases:
\begin{enumerate}
\item Event driven spike delivery, during which the callback function of each synapses activated by a spike at a given timestep is called
\item Matrix assembly, during which the $I_{ion}$ and $I_{syn}$ contributions are computed and included in the matrix
\item Matrix resolution, during which the membrane potential for the current step is obtained by solving a linear system
\item State variables update, during which the evolution equations for the states of ion channels and synapses are solved to advance to the current timestep
\item Threshold detection, during which each neuron is sca-nned to see if it has met a particular firing condition, and if so a particular list of events is updated
\item Spike exchange, during which the list of synaptic events is synchronised across all relevant neurons
\end{enumerate}
A common optimization of this algorithm makes use of the concept of minimum network delay, which requires the last step to be performed only a certain number of time steps. A representation of the six phases that were just described is given in Figure~\ref{fig:workflow}. \par
\begin{figure}
\centering
\resizebox{!}{0.35\textheight}{\input{WorkflowDiagramNew.tex}}
\caption{Workflow of a hybrid clock-event driven algorithm for the compartmental modeling of neurons.\label{fig:workflow}}
\end{figure}





